Relational structures of fundamental theories

General relativity and quantum mechanics have both revealed the relativity of certain notions that were previously thought to be absolute. I clarify the precise sense in which these theories are relational, and I argue that the various aspects of relationality pertain to the same movement in the progress of physical theories.

==> config.tex <==

\usepackage{graphicx}
\usepackage{float}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage[colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue, breaklinks=true]{hyperref}
\usepackage{breakurl}

\usepackage{comment}

\usepackage{bbold}
\usepackage{physics} % for \bracket \matrixel \Re \Im
\usepackage[percent]{overpic} %writing over pictures

% for english language
\usepackage[english]{babel}

% for quotation marks (english style)
\usepackage[autostyle, english = british]{csquotes}
\MakeOuterQuote{"}

% doi links in references
\RequirePackage{doi}

% colour comments
\usepackage[dvipsnames]{xcolor}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}

